Optimistic Policy Optimization is Provably Efficient in Non-stationary MDPs

We study episodic reinforcement learning (RL) in non-stationary linear kernel Markov decision processes (MDPs). In this setting, both the reward function and the transition kernel are linear with respect to the given feature maps and are allowed to vary over time, as long as their respective parameter variations do not exceed certain variation budgets. We propose the \underline{p}eriodically \underline{r}estarted \underline{o}ptimistic \underline{p}olicy \underline{o}ptimization algorithm (PROPO), which is an optimistic policy optimization algorithm with linear function approximation. PROPO features two mechanisms: sliding-window-based policy evaluation and periodic-restart-based policy improvement, which are tailored for policy optimization in a non-stationary environment. In addition, only utilizing the technique of sliding window, we propose a value-iteration algorithm. We establish dynamic upper bounds for the proposed methods and a minimax lower bound which shows the (near-) optimality of the proposed methods. To our best knowledge, PROPO is the first provably efficient policy optimization algorithm that handles non-stationarity.

==> regret.tex <==
\section{Regret Analysis}
In this section, we establish an upper bound of regret of Model-Based OPPO  (Algorithm \ref{alg:1}) in the following theorem. 

Our analysis relies on the following two assumptions.


\begin{assumption} \label{assumption:feature}
	There exists positive parameters $C_M$, $C_\eta$, $C_\psi$ and $C_\psi'$ such that \\
	$
	\begin{array}{l}\text { 1. }\left\|M^{*}\right\|_{F}^{2} \leq C_{M} \cdot d \\ \text { 2. } \forall(s, a) \in \mathcal{S} \times \mathcal{A}: \quad\|\eta(s, a)\|_{2}^{2} \leq C_{\eta} d \\ \text { 3. } \forall v \in \mathbb{R}^{S}: \quad\left\|\Psi^{\top} v\right\|_{\infty} \leq C_{\psi}\|v\|_{\infty}, \quad \text { and } \quad\left\|\Psi K_{\psi}^{-1}\right\|_{2, \infty} \leq C_{\psi}^{\prime}.\end{array} 
	$
\end{assumption}
See \cite{yang2019reinforcement}.


\begin{assumption} \label{assumption:tv}
	There exists a constant $B_{TV} > 0$ such that $\sum_{k=1}^K \| \theta_h^{k-1} - \theta_h^k \|_2 \le B_{TV}$ for any $h \in [H]$.
\end{assumption}
See \cite{besbes2014stochastic, russac2019weighted}.









\begin{theorem} \label{thm:regret}
	Suppose Assumptions \ref{assumption:linear:reward}, \ref{assumption:transition}, \ref{assumption:feature}, and \ref{assumption:tv} hold. Let $\alpha = \sqrt{2 \log | \cA | /H^2K}$ and $\beta_k' \geq c (C_M + {C_\psi'}^2) \cdot \log (2kHC_\eta/p)\cdot d$ for some sufficiently large constant $c>0$. Assuming that $\log | \cA | = \cO\bigl(d^3 \cdot  \log(T)^2 \bigr)$,  we have 
	\$
	Regret(T) \le \cO(dT) + \cO\bigl(\log(T) \cdot \sqrt{d^3H^3T}\bigr)
	 \$ 
	with probability at least $1-p$.
\end{theorem}
\begin{proof}
	See Section \ref{sec:sketch} for a proof sketch and Appendix \ref{appendix:proof:regret} for a detailed proof.
\end{proof}










